Semi-Cyclic Stochastic Gradient Descent

We consider convex SGD updates with a block-cyclic structure, i.e. where each cycle consists of a small number of blocks, each with many samples from a possibly different, block-specific, distribution. This situation arises, e.g., in Federated Learning where the mobile devices available for updates at different times during the day have different characteristics. We show that such block-cyclic structure can significantly deteriorate the performance of SGD, but propose a simple approach that allows prediction with the same performance guarantees as for i.i.d., non-cyclic, sampling.

==> arXiv submission/header.tex <==
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{color}

% \usepackage[numbers]{natbib}
% \bibliographystyle{plainnat}

\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\!\left[{#1}\right]}
\newcommand{\Ee}[2]{\E_{{#1}}\!\left[{#2}\right]}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\abs}[1]{\left\lvert{#1}\right\rvert}
\newcommand{\R}{\mathbb{R}}
\DeclareMathOperator\spn{span}

\definecolor{darkgreen}{rgb}{0,0.4,0.0}
\newcommand{\mcmahan}[1]{[{\color{red}{\textbf{Brendan:} \emph{#1}}}]}
\newcommand{\natinote}[1]{[{\color{magenta}{\textbf{Nati:} \emph{#1}}}]}
\newcommand{\knote}[1]{[{\color{blue}{\textbf{Kunal:} \emph{#1}}}]}
\newcommand{\tknote}[1]{[{\color{cyan}{\textbf{Tomer:} \emph{#1}}}]}
\newcommand{\huberte}[1]{[{\color{green}{\textbf{Hubert:} \emph{#1}}}]}

\newcommand{\removed}[1]{}
\usepackage{soul}
\newcommand{\maybe}[1]{{\color{yellow}{#1}}}

\newenvironment{question}[1]{\paragraph{Open Question: #1}\begin{em}}{\end{em}}



